Chain-of-Model Learning for Language Model

In this paper, we propose a novel learning paradigm, termed Chain-of-Model (CoM), which incorporates the causal relationship into the hidden states of each layer as a chain style, thereby introducing great scaling efficiency in model training and inference flexibility in deployment. We introduce the concept of Chain-of-Representation (CoR), which formulates the hidden states at each layer as a combination of multiple sub-representations (i.e., chains) at the hidden dimension level. In each layer, each chain from the output representations can only view all of its preceding chains in the input representations. Consequently, the model built upon CoM framework can progressively scale up the model size by increasing the chains based on the previous models (i.e., chains), and offer multiple sub-models at varying sizes for elastic inference by using different chain numbers. Based on this principle, we devise Chain-of-Language-Model (CoLM), which incorporates the idea of CoM into each layer of Transformer architecture. Based on CoLM, we further introduce CoLM-Air by introducing a KV sharing mechanism, that computes all keys and values within the first chain and then shares across all chains. This design demonstrates additional extensibility, such as enabling seamless LM switching, prefilling acceleration and so on. Experimental results demonstrate our CoLM family can achieve comparable performance to the standard Transformer, while simultaneously enabling greater flexiblity, such as progressive scaling to improve training efficiency and offer multiple varying model sizes for elastic inference, paving a a new way toward building language models. Our code will be released in the future at: https://github.com/microsoft/CoLM.

==> sections/experiments/settings.tex <==
\subsection{Experimental Setting}
\label{subsec:experimental_setting}
In our experiments, we utilize the SlimPajama dataset~\cite{cerebras2023slimpajama} as the pre-training corpus, comprising 627 billion tokens. Here, we use LLama-2-tokenizer~\footnote{\url{https://huggingface.co/meta-llama/Llama-2-7b}} to process corpus, with a vocab size of 32000. We leverage Fully Sharded Data Parallel (FSDP2) for distributed training, facilitated by the TorchTitan framework~\cite{Wanchao2024TorchTitan}. Our training is built upon a cluster of 32 NVIDIA A100 40GB GPUs with a gradient accumulation of 4, yielding an effective batch size of 1024. We adopt the mixed precision by using BFloat16. Our CoLM is pre-trained with a sequence length of 4096 tokens, by using AdamW optimizer~\cite{Diederik2015Adam} with a learning rate of $1.5\times10^{-4}$. FlashAttention-2~\cite{Tri2024FlashAttention2} is applied to speed up attention computation. More experimental details can refer to Appendix~\ref{appendix:experimental_details}.
